The Weighted Euler Characteristic Transform for Image Shape Classification

The weighted Euler characteristic transform (WECT) is a new tool for extracting shape information from data equipped with a weight function. Image data may benefit from the WECT where the intensity of the pixels are used to define the weight function. In this work, an empirical assessment of the WECT's ability to distinguish shapes on images with different pixel intensity distributions is considered, along with visualization techniques to improve the intuition and understanding of what is captured by the WECT. Additionally, the expected weighted Euler characteristic and the expected WECT are derived.

==> body/declarations.tex <==
\section*{Declarations}

\paragraph{Funding}
JCK and BTF acknowledge support from NSF under Grant Numbers DMS 2038556 and 1854336.
BTF and EQ also acknowledge support from NSF under Grant Number 1664858.

\paragraph{Conflicts of interest/Competing interests}
The authors declare that they have no conflicts of interest.

\paragraph{Availability of data and material} Not applicable.

\paragraph{Code availability} The code related to this project will be available at \url{https://github.com/compTAG/image-wect}.

\paragraph{Authors' contributions}
Drs. Cisewski-Kehe and Fasy co-directed this research.  Dhanush Giriyan worked as a summer intern, where he worked on a preliminary version of the results and contributed to an initial write-up, which he presented at the Young Researcher's Form (which had no formal proceedings).  Eli Quist contributed to editing that codebase, running all the experiments, and summarizing the experimental results.

\paragraph{Additional declarations for articles in life science journals that
report the results of studies involving humans and/or animals} Not applicable.

\paragraph{Ethics approval} Not applicable.

\paragraph{Consent to participate} Not applicable.

\paragraph{Consent for publication} If accepted, the publication of this
manuscript is accepted by all coauthors.


==> body/init.tex <==



